Data-Driven Characterization and Detection of COVID-19 Themed Malicious Websites

COVID-19 has hit hard on the global community, and organizations are working diligently to cope with the new norm of "work from home". However, the volume of remote work is unprecedented and creates opportunities for cyber attackers to penetrate home computers. Attackers have been leveraging websites with COVID-19 related names, dubbed COVID-19 themed malicious websites. These websites mostly contain false information, fake forms, fraudulent payments, scams, or malicious payloads to steal sensitive information or infect victims' computers. In this paper, we present a data-driven study on characterizing and detecting COVID-19 themed malicious websites. Our characterization study shows that attackers are agile and are deceptively crafty in designing geolocation targeted websites, often leveraging popular domain registrars and top-level domains. Our detection study shows that the Random Forest classifier can detect COVID-19 themed malicious websites based on the lexical and WHOIS features defined in this paper, achieving a 98% accuracy and 2.7% false-positive rate.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> recommendations.tex <==

This section summarizes the experts' recommendations provided by industry leaders and our independent tips on maintaining enterprise security, privacy regulation compliance and business continuity during this pandemic and similar future extended period of business disruption. We compile a separate list of recommendations based on `stay-at-home' (or WFH policy) orders in effect or not.
%{\color{blue} We also discuss the feasibility and importance of executing recommended actions in organizations based on their sizes?}

%\subsection{Recommendations from Experts Regarding Remote Work}

\subsection{Recommendations Regarding Remote Work}
Since COVID-19 disease has no vaccination yet, to slow down the infection rate, stay-at-home orders along with social distancing have been the most effective ways to allow health systems to treat COVID-19 patients without overwhelming their resources \cite{Stay_home_covid19}. Thus, while assessing the cybersecurity plans for business continuity, enterprises need to keep WFH policy in mind. During active WFH policy enterprises should publish clear guidelines for their remote employees. The following recommendations can guide the community to chose from according to their budgets and valuation of assets. 
%\subsubsection{Secure home networks}
\subsubsection{Secure home-work environments}
\begin{recommendation}
Practice ``digital distancing" by setting up routers with two separate networks, isolate enterprise networks from unpatched home devices  \cite{CBDigitalDistancing}.
\end{recommendation}

\begin{recommendation}
Enterprises should provide tips to secure home networks and deliver security updates outside of corporate networks \cite{CBDigitalDistancing}.
\end{recommendation}

\begin{recommendation}
Provide employees with work laptops at home to have all the essential standard tools in that machine readily available, it can protect enterprises from reducing attack surfaces created by unverified and unchecked third-party software installations at employee's end. 
\end{recommendation}

\begin{recommendation}
\label{rec:dnsSettingsPass}
Provide guidelines for employees and customers to use stronger passwords for PCs and routers, regularly monitor DNS settings. 
\end{recommendation}

\begin{recommendation}
Build capabilities of enterprise threat hunting within employee's home network environments \cite{CBDigitalDistancing}.
\end{recommendation}
\subsubsection{Do not neglect employee information and privacy}
\begin{recommendation}
Record only factual information and  minimum amount of information necessary. 
\cite{Addiscott2020}.
\end{recommendation}
%disucssion points
%Experts from VMware Carbon Black, a top giant in the cybersecurity industry, have published an on-demand webinar discussion where they metaphorically presented ``digital distancing" as equivalent to ``social distancing" while fighting against the unprecedented cyberattacks during this pandemic in the digital world . 
%They bring the fact that many of our smart devices at home are unpatched. While 80-90\% percent of employees are working from home, they are making the enterprise network vulnerable by increasing the attack surface that is not in sight of any security teams. Given these facts they recommends the following to reduce the attack surface.

\subsubsection{Secure remote communication}
\begin{recommendation}
Always use passwords and restrict user joining meetings by admin verification for remote meetings to avoid any eavesdropping \cite{CBDigitalDistancing}. 
\end{recommendation}

\begin{recommendation}
Do not use keywords such as `sensitive', `secret', `highly-classified' as meeting titles \cite{CBDigitalDistancing}.
\end{recommendation}

\begin{recommendation}
Leveraging virtual private networks (VPN) for remote access to enterprise network while working from home \cite{CBWashingHand20s}.
\end{recommendation}

\begin{recommendation}
\label{rec:mfa}
Using multi-factor authentication (MFA) for all critical communications and transactions \cite{CBWashingHand20s}. (more citations) 
\end{recommendation}

%The session also recommended to practice organizational security hygiene as listed below -
\subsubsection{Build more informed users}
\begin{recommendation}
Enterprise should specify a (or make a white-list) VPN software and remote access tools for their employees which may prevent them falling into VPN lure traps.
\end{recommendation}

\begin{recommendation}
Provide clear direction for remote meeting software and meetings norms while working from home.
\end{recommendation}

\begin{recommendation}
Enterprise should provide specific guidelines for employees and consumers to securely access data and networks remotely.
\end{recommendation}


%Next, another cybersecurity expert from VMware Carbon Black, recommended three necessary steps as equivalent to ``washing your hands for the 20 seconds" to protect enterprise security \cite{CBWashingHand20s}. These steps are listed as the next three subsequent recommendations below. 
%These same set of recommendations are also coming from other security experts and farms \cite{}. The steps are listed below as individual recommendations. 







%Experts suggest that train employees are still one of the most effective ways to fight against these large number of attacks. Thus, early warnings and communications about similar attack scenarios and implementing policies on what to do with such COVID-19 related emails should be in place \cite{CyberHyigene_during_COVID19}.


%Finally, experts suggests enterprises to have a compact and immediate incident response plan if COVID-19 related security breach happens during this pandemic.



%avoid online viruses by virtual social distancing: (don't right away believe what you see or read, it may be a misinformation, check source, check publish date, search other media that publishes similar story...) report in https://siliconangle.com/2020/04/03/cyber-hygiene-in-the-time-of-covid-19-avoid-catching-an-online-virus-by-virtual-social-distancing-cubeconversations/


%\subsection{Recommendations on enterprise security while `stay-at-home' orders in place}
%\subsubsection{Technical safeguards}


%These whitelisting of applications would provide more visibility from the defenders' perspective. 






%Another essential advice is to strengthen the remote access policies of the enterprise as remote working might be a ``new normal" for the rest of this year 2020. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Recommendations from Experts Independent of Remote Work}
\subsection{Recommendations Independent of Remote Work}
Though WFH policy is the actual reality in many industries at current situation, COVID-19 themed attacks may stay even longer after the stay-at-home orders are lifted. 
%Mass campaigns with email lures, building \& registering malicious domains, creating malicious mobile applications can still impact the businesses which are already hardly impacted economically. 
Hence to be resilient during this crisis and future similar themed cyberattacks there is no other alternative than practicing standard cyber hygiene, be vigilant, and establish more proactive defense strategies. The list of recommendations are as follows.

\subsubsection{Secure end-points}
%Thus enterprises need guidelines for secure business continuity to fight this pandemic from both health and economic perspectives.  
\begin{recommendation}
Timely patching and updating of all software and operating systems \cite{CBWashingHand20s}.
\end{recommendation}


\subsubsection{Secure networks \& systems}
\begin{recommendation}
Using mandatory passwords for changing any application settings, if working with sensitive infrastructures, system level whitelisting of applications can be practiced \cite{CBDigitalDistancing}. 
\end{recommendation}

%\subsubsection{Improve security practices}


%\subsubsection{Secure }
\begin{recommendation}
Establish proactive defense against COVID-19 related malicious and abused websites, domains, URLs, and IP addresses.
\end{recommendation}

\begin{recommendation}
Establish proactive defense against COVID-19 themed malicious emails through scanning and reviewing emails with COVID-19 related subject, body, links, and attachments before sending it to employee's inbox.  
\end{recommendation}

\subsubsection{Build more informed users}
\begin{recommendation}
Enterprise should establish a secure communication channel either through email or web portal for reliable COVID-19 related information and updates, try to boost employee morale by showing more connection and compassion.  
\end{recommendation}

\begin{recommendation}
\label{rec:awareOnlure}
Establish an effective way to regularly communicate about new COVID-19 related lures, misinformation, myths, and risk factors to employees and customers to educate them beforehand \cite{CBDigitalDistancing}.
\end{recommendation}

\begin{recommendation}
Train employees to be skeptical and vigilant about emails with COVID-19 related updates, information, guidelines, or about ongoing sales or deals.
\end{recommendation}

\begin{recommendation}
Encourage and provide guidelines for employees and customers to report about any suspicion, scams, or abuses to IT (or security) teams.   
\end{recommendation}

%\begin{recommendation}
%Organizations should warn their employees to be skeptical about COVID-19 related emails with links and attachments from the company’s CEO, personal doctors with COVID-19 advice and guidelines, or emails pretending to be deals/offers from legit retailers. \cite{}
%\end{recommendation}


%\begin{recommendation}
%Employees should be trained not to open suspicious emails, not to click on attachments or links, and know the steps on what to do or whom to notify when they encounter such an email.
%\end{recommendation}


%\begin{recommendation}
%Everyone should always double-check the %sender's address for COVID-19 emails to %catch email masquerading.
%\end{recommendation}


%\begin{recommendation}
%Instead of making payments from email links, users should go to the original source website when donating to a COVID-19 cause. 
%\end{recommendation}

\subsubsection{Coordinated cyber security management}
\begin{recommendation}
Security teams should coordinate with decision-makers to setup a compact incident response plans by following standard NIST cybersecurity framework \cite{NIST_framework} against any successful COVID-19 themed attacks. 
\end{recommendation}

\begin{recommendation}
Enterprises should be proactive and adapt to fast changes regarding existing models and frameworks to detect new COVID-19 attacks.
\end{recommendation}


\begin{recommendation}
Maintain cyber hygiene by checking reviews of software before use and discuss new software pros and cons among peers.
\end{recommendation}

%\begin{recommendation}
%Enterprises can encourage their employees to check news and COVID-19 updates only from authorized and reliable sources to avoid misinformation dissemination. They can compile those information sources and share with their employees. 
%\end{recommendation}


%\begin{recommendation}
%Double-checking website addresses may protect individuals either from visiting a typo-squatting and/or visually similar phishing website, or from downloading malware.
%\end{recommendation}


%\begin{recommendation}
%Employees should act responsibly, and they should verify from reliable sources before sharing sensitive news with other colleagues.
%\end{recommendation}


%\begin{recommendation}
%(May not be in scope?) Internet users should not buy or trust testing kits, vaccines, therapies, cures from unreliable sources that are not approved by national or international level health agencies.
%\end{recommendation}



%predicting known attack groups from real-time incident reports and security logs,

%\subsubsection{Awareness safeguards} 
%Moreover, enterprises should actively communicate these risk factors and attack scenarios to train their employees and users. 

%Primarily, All enterprises should communicate their employees on how often and who are going to send emails regarding COVID-19. 
%Suspicious emails may use COVID-19 lures (mentioned in section 3) to emotionally distressed employees with compassionate sentences to become successful. 

%The first wall of defense is the human shield, as most of the attacks need human interaction and error to be victorious. 
%Enterprises should teach their employees on hidden email links and how hovering over a link can discover the real website (or domain address). 

%We should not download untrusted third-party VPN, remote access, and virtual meeting software. 

 
\subsection{Recommendations Against Rising Non-COVID-19 Themed Cyberattacks}
Along with the rise in COVID-19 themed cyber attacks as discussed in section \ref{sec:methodology}, we are also observing other state-of-the-art non-COVID-themed attacks gaining recent interest because of added incentives amid COVID-19 pandemic. We are listing those attacks as we understand being informed and vigilant as a community can help us stay safe. 
\subsubsection{Ransomware attacks}
Ransomware is a special kind of malware and propagates similarly through websites, emails, and mobile applications. Thus, securing this artifacts may also provide proactive security against ransomware attacks as well. However, some advanced multi-stage attacks (APTs) may target healthcare and COVID-19 research facilities with ransomware attacks. Compliance with standard cyber hygiene and best security practices should keep enterprise safe from ransomware attacks \cite{CISA_ransomware, hornetsec_ransomware}. Moreover, enterprise should be vigilant about new zero-day CVEs and software vulnerabilities to keep their enterprise network safe.

\subsubsection{Impersonation attacks}
Since COVID-19 pandemic force us to go virtual for business continuity, it creates opportunity for attackers to impersonate as legitimate entities (e.g., government, doctor, CEO, WHO) and make fraud transactions, compromise business emails, and other similar attacks. Usually, impersonation attacks are carried out through emails, chats, phone calls, and SMSs. As per recommendations \ref{rec:mfa} and \ref{rec:awareOnlure}, enterprises should inform their employees on such lures and enforce MFA for all critical transactions and communications during this pandemic. 

%Enterprises also need to communicate these scenarios well ahead so that their customers and employees are aware and do not fall victim to such social engineering attacks. 
%Moreover, fraud donation websites and payment links in email for COVID-19 donations, claiming to support WHO or similar organizations who are fighting from the frontline can be detected by checking the payment methods. If the donation campaigns did not allow users to pay through credit card or PayPal (and similar) payment system instead asking for bank transfers should is a clear indicator of donation scamming. 

\subsubsection{Defense against router DNS hijacking}
Router DNS hijackings are attacks where attackers get remote access to routers and change DNS settings to land victims into attacker controller websites and launch malware or phishing attacks. We have seen reports on these attacks rising during COVID-19 as with active WFH policies attackers have far more incentive than regular times \cite{oski_malware_attack_covid19}. The most effective defense against router DNS hijacking is to practise recommendation \ref{rec:dnsSettingsPass} \cite{DNS_hijack_protection}. Additionally, defenders can raise alerts if the browser automatically redirects from a reputed website to a non-reputed ones because of change in the DNS settings. 

\subsubsection{Defense against Zoom-bombing attacks}
Zoombombing is when an unauthorized person or stranger joins a Zoom meeting/chat session and cause disorder by saying offensive things and even photobombing the meeting by sharing pornographic and hate images. When using Zoom for online classrooms, meetings or events, the host is advised to making meetings private and require a password or use the waiting room feature to control the admittance of additional people.  The links to a teleconference or classroom should be sent directly to the individual participants and never be publicly available on a social media post.  Turn off the annotation feature and restrict other feature as needed in host controls. Those managing a conference in Zoom should change the screen sharing option to “Host-Only.” Finally, you should always run the latest version of Zoom.

\subsubsection{Defense against HTML/XSS injection attacks}
Website and mobile app injections attacks are handy during a pandemic to propagate various malware. These attacks can be far more impactful when injected into a top legitimate website working for COVID-19 related data and updates with large volume of live users. Hence, such organization and website should regularly scan and check for changes in their website HTML contents, added scripts, hidden divisions, and images. 

\ignore{
{\color{red}\footnote{find an appropriate home for this paragraph. I think we can use this as part of the discussion/conclusion to make a final comment on the issue ...}
%discussion on implementing zero-trust securitymodel
VPN alone would not be enough, and large scale use of VPNs may provide enough incentives to attackers for targeting their attacks for VPN vulnerabilities \cite{CyberHyigene_during_COVID19}. We also find discussion from experts \cite{zero_trust_model_for_COVID_cw, zero_trust_model_for_COVID_dr, zero_trust_model_for_COVID_ng} suggesting more stringent approach to implement zero-trust security models \cite{zero_trust_model_citrix, zero_trust_model_cloudflare, zero_trust_model_cso} for enterprise data and network access. This pandemic should give the enterprise leaders a strong message to strengthen security monitoring, proactive defense, and test security software effectiveness regularly.
}}
%These can be summarized from the various website ...
%\subsection{Recommendations Specific to Incidents}

%\subsubsection{Generic Recommendations When There Is No "Stay at Home" Policy}

%e.g., what if it's political event?

%\subsubsection{Generic Recommendations When There Is  "Stay at Home" Policy}

%e.g., what if it's COVID-XX?

